Unified Framework for Open-World Compositional Zero-shot Learning

Open-World Compositional Zero-Shot Learning (OW-CZSL) addresses the challenge of recognizing novel compositions of known primitives and entities. Even though prior works utilize language knowledge for recognition, such approaches exhibit limited interactions between language-image modalities. Our approach primarily focuses on enhancing the inter-modality interactions through fostering richer interactions between image and textual data. Additionally, we introduce a novel module aimed at alleviating the computational burden associated with exhaustive exploration of all possible compositions during the inference stage. While previous methods exclusively learn compositions jointly or independently, we introduce an advanced hybrid procedure that leverages both learning mechanisms to generate final predictions. Our proposed model, achieves state-of-the-art in OW-CZSL in three datasets, while surpassing Large Vision Language Models (LLVM) in two datasets.

==> experiment/experiment_closed.tex <==
\subsection{Results on Closed World Setting}
In order to measure the flexibility of proposed model, we conduct experiments on closed world setting. During the evaluation we adjust the feasibility mask to represent total number seen and unseen pairs present in the dataset. This transition the proposed model from open world setting to closed world setting. 
\bgroup
\def\arraystretch{1.2}
\begin{table}[h]
\setlength\tabcolsep{3pt}
\caption{Closed world performance on MIT-States, C-GQA and VAW-CZSL. As evaluation matrices we refer to AUC with seen and unseen accuracies and HM.}
\begin{center}
\fontsize{6.5}{9}\selectfont 
\label{tab:results_close}
\begin{tabular}{l c c c c|c c c c|c c c c}
Method  & \multicolumn{4}{c|}{MIT-States} & \multicolumn{4}{c|}{C-GQA} & \multicolumn{4}{c}{VAW-CZSL} \\
& S & U  & HM  & AUC & S & U  & HM  & AUC& S & U  & HM  & AUC\\
\cline{2-13}
CGE$_{vit}$\cite{naeem2021learning}& 39.7  & 31.6 & 24.8 & 9.7 & 38.0 & 17.1  & 18.5  & 5.4& 30.1 & 25.7  & 20.1  & 6.2\\
OADIs$_{vit}$\cite{Saini2022Disentangling} & 39.2  & 32.1 & 25.2 & 10.1 & 38.3 & 19.8 & 20.1  & 7.0& 31.3 & 26.1 & 20.4 & 6.5\\
CoT$_{vit}$\cite{kim2023hierarchical} & 39.5 & 33.0 & 25.8 & 10.5 & 39.2& 22.7 & 22.1 & 7.4& 32.9& 28.2 & 21.7 & 7.2\\
% $\mathbb{CSP}$\cite{nayak2022learning}&closed& 46.6  & 49.9  & 36.3 &  19.4  &  &  &  &  &  &  &  & \\
% \cdashline{1-14}
% KG-SP$_{vit}$\cite{karthik2022kg}&open&   &  &  &  &  &   &   & &  &  &   & \\
% $\mathbb{CSP}$\cite{nayak2022learning}&open&   &  &  &  &  &  &  &  &  &  &  & \\
\cline{1-13}
Ours$_{vit}$& 36.5  & 30.9 & 22.1 & 8.2 & 36.1  &  18.7  &  19.3 & 5.8 & 17.1  &  14.2  &  10.3  & 1.8 \\
\cline{1-13}
\end{tabular}
\end{center}
\end{table}
\egroup

\noindent Proposed model able to achieve competitive results on all datasets while deploying in much larger output space.

==> feasibility.tex <==
% Feasibility score is computed by evaluating if a given attribute object composition makes sense in the real world or not. For example, 'small cat' is makes sense while 'spilled cat' dose not make sense. 
Feasibility score is determined by assessing the coherence of attribute-object compositions within real-world contexts. For example, while 'small cat' exhibits coherence, 'spilled cat' lacks semantic coherence. This aims to ascertain the viability of a given attribute-object pair within real-world contexts. In order to compute the feasibility scores for each composition, we deploy a similar procedure as KG-SP\cite{karthik2022kg}. First, we aggregate text embedding for each word in the vocabulary by utilizing GloVe \cite{pennington2014glove}. Subsequently, we find similarity between given object and available objects and computing similarity scores for attributes as well. Lastly, for each composition, a feasibility score, $\rho_{Glove}(a,o) \in \mathbb{R}$ is calculated by taking the average of similarity scores between respective attribute and object.
\begin{align}
\rho_o(a,o) &=\max_{\hat{o}\in\mathbb{O}}\frac{\phi(o)\cdot\phi(\hat{o})}{||\phi(o)||\cdot||\phi(\hat{o})||}\\
\rho_{Glove}(a,o) &=\frac{\rho_o(a,o)+\rho_a(a,o)}{2}
\end{align}
Where, $\rho_o(a,o)$ is the maximum similarity score between object and other objects in $\mathbb{O}$. $\phi(\cdot)$ is the GloVe embedding function. In order to induce more robustness to the filtering, we compute ConceptNet numberbatch \cite{speer2017conceptnet} embedding based feasibility scores similar to that of Glove. For each pair, maximum of two feasibility scores set as the final feasibility score $\rho(a,o)\in \mathbb{R}$.
\begin{align}
\rho(a,o) &=\max_{o\in\mathbb{O},a\in\mathbb{A}}(\rho_{Glove}(a,o) ,\rho_{Conceptnet}(a,o) )\\
f_{pair} &=\operatorname*{arg\,max}_{y,\rho(a,o)>T} p_{\theta}(y|x)
\end{align}
Where, $\rho(a,o)$ is the feasibility score for composition $(a,o)$. Finally, we filter out the infeasible compositions by choosing the compositions with higher scores than a empirically settled threshold value which is calibrated on training set. Resulting a binary mask $f_{pair} \in \mathbb{R}^{|A|\cdot|O|}$.

% \newpage
\subsection{Feasibility Results}
We examine the least and most feasible attribute-object combinations computed within the MIT-States validation set. Subsequently, we compare the associated labels and corresponding predictions. Column one displays corresponding image, with the ground-truth label positioned at the top (GT), while columns two and three shows attribute and object predictions. Furthermore, fourth column consists of incorrect predictions. Last column indicate the final pair prediction. For each cell, three columns illustrate the top-3 results for attributes, objects, and compositions. We denote the predictions matching the ground truth are highlighted in blue. 

From Table \ref{fig:multi1} it is evident that, compositions with lower feasibility scores are susceptible to masking out thereby introducing an induced bias within the network and consequently resulting in incorrect predictions. In contrast, Table \ref{fig:multi2} illustrates the model's capability to accurately identify labels for compositions with higher feasibility scores. Consequently, this highlights the model's ability to discern such compositions without the risk of masking out. 
% Consequently, these compositions do not introduce masking-off dangers, thereby enhancing the network's predictive accuracy.
% On the other hand, Table \ref{fig:multi1} shows that the model being able to recognize correct labels for compositions with higher feasibility scores. As the model definitely sees these compositions as they don't have a danger in masking off.
Therefore, above results prompt us to explore novel methodologies to compute more robust and scalable feasibility scores. Such that it would encompass a right-skewed distribution to accurately represent viable compositions. 
% that will include right skewed distribution for viable compositions.
% [(('bent', 'gate'), tensor(0.2094)), (('deflated', 'pool'), tensor(0.1847)), (('engraved', 'key'), tensor(0.1964)), (('peeled', 'tiger'), tensor(0.1524)), (('rusty', 'penny'), tensor(0.1352)), (('squished', 'mud'), tensor(0.1938)), (('steaming', 'horse'), tensor(0.1735)), (('torn', 'jungle'), tensor(0.1882))]


==> multiple_objects.tex <==
% \subsubsection{Identifying Multiple Object Instances}
\begin{table}[h]
\setlength\extrarowheight{2pt} % for a more open "look"
\centering
\tiny
\caption{Performance of the model in the presence of multiple object instances. Secondary object predictions are highlighted in \wrong{red} and final predictions are highlighted with black boxes.}\label{fig:multi}
\begin{tabular}{C{0.75cm} C{0.3cm} C{0.001cm}C{0.75cm} C{0.75cm} C{1.4cm} | C{0.75cm} C{0.3cm} C{0.001cm}C{1.1cm} C{0.75cm} C{1.4cm} }
  % \cline{1-6}  
  \multicolumn{3}{c}{GT: Huge Bear}
  &&&&\multicolumn{3}{c}{GT: Stone Stairs}\\

  \multicolumn{3}{c}{\multirow{3}{*}{\centering\includegraphics[width=0.13\linewidth, height= 1cm]{fig/multiple_1.jpg}}}&\boxit{1.25in}\scalebox{.8}{\text{\correct{huge}}}&\scalebox{.8}{\text{\correct{bear}}}&\scalebox{.8}{\text{\correct{huge bear}}}
  &\multicolumn{3}{c}{\multirow{3}{*}{\centering\includegraphics[width=0.13\linewidth, height= 1cm]{fig/multiple_2.jpg}}}&\boxit{1.6in}\scalebox{.8}{\text{\wrong{skateboarding}}}&\scalebox{.8}{\text{\wrong{jeans}}}&\scalebox{.8}{\text{\wrong{skateboarding boy}}}\\

% \addlinespace[-1ex]
  &&&\scalebox{.8}{\text{\wrong{mossy}}}&\scalebox{.8}{\text{dog}}&\scalebox{.8}{\text{young bear}}
  &&&&\scalebox{.8}{\text{\wrong{skating}}}&\scalebox{.8}{\text{boy}}&\scalebox{.8}{\text{\wrong{skateboarding man}}}\\

  % \addlinespace[-1ex]
  &&&\scalebox{.8}{\text{young}}&\scalebox{.8}{\text{\wrong{forest}}}&\scalebox{.8}{\text{mossy bear}}
  &&&&\scalebox{.8}{\text{\wrong{black}}}&\scalebox{.8}{\text{man}}&\scalebox{.8}{\text{\wrong{jumping boy}}}\\ 
  % \cline{1-6}
\end{tabular}
\end{table}
In Table \ref{fig:multi}, we examine the model's capability in managing multiple object instances. For column 1, model successfully recognized both `bear' and `forest' while giving priority for `bear' during predictions. However in column 2, predictions are predominantly influenced by secondary objects: `skateboarding' and clothing. Thus demonstrating the model's capability to identify diverse set of object instances.

